Neutral hydrogen filaments in interstellar media: Are they physical?

The trending term "filament" is extensively used in the interstellar medium (ISM) and the star formation community, and is believed to be one of the most important objects that gauge molecular cloud and star formation. However, the physical definition of these ubiquitous, elongated, high contrast features is poorly defined and still actively debated. Despite the absence of a unified consensus, filaments are believed to be involved in many important physical processes from galaxy structure formation to the emergence of protostellar objects. Therefore, understanding how filaments form, what constrains their growth, and their general physical properties, are extremely important for theorists and observers who study the dynamics of the ISM and consequent star formations. This review serves as a collection of the community's views and develops the concept of "filaments" in the context of the ISM and star-forming clouds. Observationally, filaments are seen across the entire sky and often carry an aspect ratio of the order of hundreds. In the context of the ISM, filaments are believed to form by stretching and tearing from magnetized ISM turbulence. ISM filaments are subjected to heating and cooling phases, and are likely to be magnetically aligned. Cold clouds are formed inside ISM due to turbulence instability. This review updates the understanding of ISM filaments in the community.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


